NaViL: Rethinking Scaling Properties of Native Multimodal Large Language Models under Data Constraints

Compositional training has been the de-facto paradigm in existing Multimodal Large Language Models (MLLMs), where pre-trained vision encoders are connected with pre-trained LLMs through continuous multimodal pre-training. However, the multimodal scaling property of this paradigm remains difficult to explore due to the separated training. In this paper, we focus on the native training of MLLMs in an end-to-end manner and systematically study its design space and scaling property under a practical setting, i.e., data constraint. Through careful study of various choices in MLLM, we obtain the optimal meta-architecture that best balances performance and training cost. After that, we further explore the scaling properties of the native MLLM and indicate the positively correlated scaling relationship between visual encoders and LLMs. Based on these findings, we propose a native MLLM called NaViL, combined with a simple and cost-effective recipe. Experimental results on 14 multimodal benchmarks confirm the competitive performance of NaViL against existing MLLMs. Besides that, our findings and results provide in-depth insights for the future study of native MLLMs.

==> preamble.tex <==
\usepackage{xspace}

\newcommand{\modelname}{NaViL\xspace}
% \newcommand{\modelname}{Mono-InternVL v2\xspace}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\textit{e.g}\onedot} 
\def\Eg{\textit{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} 
\def\Ie{\textit{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\usepackage{CJK}

\newcommand{\TODO}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{red}{[todo: #1]}\end{CJK}}

\newcommand{\prompt}[1]{\textcolor{black}{\footnotesize{\texttt{#1}}}}

\newcommand{\hao}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{orange}{[Hao: #1]}\end{CJK}}

\newcommand{\tcy}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{blue}{[tcy: #1]}\end{CJK}}

\newcommand{\gen}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{orange}{[Gen: #1]}\end{CJK}}

\newcommand{\zh}[1]{\begin{CJK}{UTF8}{gbsn}{#1}\end{CJK}}
\usepackage{xcolor}
% 定义自己的颜色
\definecolor{lightblue}{RGB}{152,182,234}
\definecolor{lightgreen}{RGB}{164,212,133}

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\definecolor{prompt}{rgb}{0.21,0.49,0.74}

\usepackage{array}

\usepackage[most]{tcolorbox}
\newcommand{\finding}[2]{
    % args:
    %   1: finding number
    %   2: finding text
    \vspace{-0.1cm}
    \begin{tcolorbox}[
        colback=white!90!gray,     % Soft ivory background
        colframe=teal!60!black,     % Deep navy frame color
        arc=5pt,                    % Less rounded corners for a modern look
        boxsep=5pt,                 % Inner margin between text and frame
        left=6pt,                  % Left margin within the box
        right=6pt,                 % Right margin within the box
        top=2pt,                    % Top margin within the box
        bottom=2pt,                 % Bottom margin within the box
        boxrule=0.8pt,              % Frame thickness
        drop shadow=gray!50!white,  % Subtle shadow effect for depth
        enhanced jigsaw             % Allows for the shadow effect and better arcs
    ]
    \vspace{-0.1cm}
        \paragraph{\textbf{\textit{Observation #1:}}}#2
    \vspace{-0.1cm}
    \end{tcolorbox}
    \vspace{-0.1cm}
}

\usepackage{textcomp}
